A smooth compactification of spaces of stability conditions: the case of the $A_{n}$-quiver

We propose a notion of multi-scale stability conditions with the goal of providing a smooth compactification of the quotient of the space of projectivized Bridgeland stability conditions by the group of autoequivalence. For the case of the 3CY category associated with the $A_n$-quiver this goal is achieved by defining a topology and complex structure that relies on a plumbing construction. We compare this compactification to the multi-scale compactification of quadratic differentials and briefly indicate why even for the Kronecker quiver this notion needs refinement to provide a full compactification.

==> packages.tex <==

%languages, pictures
\ProvidesPackage{language}
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{csquotes}
\usepackage{xcolor}
\usepackage{graphicx,color}
\usepackage{comment}

%biblatex
%\usepackage[style=alphabetic,backend=bibtex,maxnames=10]{biblatex}
\usepackage[style=alphabetic,
            isbn=false,
            doi=false,
            url=false,
            backend=bibtex,
            maxnames=5, 
            maxalphanames=5,giveninits=true
           ]{biblatex}
\usepackage{layout}
\usepackage{enumitem}
\usepackage{afterpage}
\usepackage{hyperref}
\usepackage{aliascnt}
%\usepackage[notref,notcite]{showkeys}
\usepackage{xparse}
\usepackage{caption}
%\usepackage{tabto}
\usepackage{imakeidx}
\usepackage[normalem]{ulem}
\allowdisplaybreaks


%math
\usepackage{amsmath,amsfonts,amsthm,mathtools,amssymb}
\usepackage{tensor}
\usepackage{amscd,latexsym, mathrsfs, epsfig}
\usepackage{mathdots}
\usepackage{upgreek}
%\usepackage{enumerate}
%\usepackage{undertilde}
\usepackage[all]{xy}

%tikz
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{float}
\usetikzlibrary{matrix,arrows,calc}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.pathreplacing,decorations.markings,decorations.pathmorphing}
\usetikzlibrary{positioning,arrows,patterns}
\usetikzlibrary{cd}
\usetikzlibrary{intersections}
\tikzset{
	every loop/.style={very thick},
	comp/.style={circle,black,draw,thin,inner sep=0pt,minimum size=5pt,font=\tiny},
	order bottom left/.style={pos=.05,left,font=\tiny},
	order top left/.style={pos=.9,left,font=\tiny},
	order bottom right/.style={pos=.05,right,font=\tiny},
	order top right/.style={pos=.9,right,font=\tiny},
	%
	order middle right/.style={draw,thin,shape=rectangle,inner sep=2pt,outer sep=5pt,pos=.5,right,font=\tiny},
	%
	order middle left/.style={draw,thin,shape=rectangle,inner sep=2pt,outer sep=5pt,pos=.5,left,font=\tiny},
	%	
	order node dis/.style={text width=.75cm},
	circled number/.style={circle, draw, inner sep=0pt, minimum size=12pt},
	below left with distance/.style={below left,text height=10pt},
	below right with distance/.style={below right,text height=10pt}
}

